ZoomOut: Spectral Upsampling for Efficient Shape Correspondence

We present a simple and efficient method for refining maps or correspondences by iterative upsampling in the spectral domain that can be implemented in a few lines of code. Our main observation is that high quality maps can be obtained even if the input correspondences are noisy or are encoded by a small number of coefficients in a spectral basis. We show how this approach can be used in conjunction with existing initialization techniques across a range of application scenarios, including symmetry detection, map refinement across complete shapes, non-rigid partial shape matching and function transfer. In each application we demonstrate an improvement with respect to both the quality of the results and the computational speed compared to the best competing methods, with up to two orders of magnitude speed-up in some applications. We also demonstrate that our method is both robust to noisy input and is scalable with respect to shape complexity. Finally, we present a theoretical justification for our approach, shedding light on structural properties of functional maps.

==> figures2/old_figures_backup.tex <==

% \begin{figure}[!t]
% \centering
% \begin{overpic}
%   [trim=0cm 0cm 0cm 0cm,clip,width=1\columnwidth]{./figures/eg_scalability_bone.png}
%   \put(3,36){\footnotesize Source}
%   \put(2,33.11){\footnotesize $n_v=5K$}
%   \put(26,36){\footnotesize Target}
%   \put(24.9,33.11){\footnotesize $n_v=1K$}
%   \put(24.9,-2){\footnotesize $t=1.25s$}
%   \put(47,36){\footnotesize Target}
%   \put(46,33.11){\footnotesize $n_v=5K$}
%   \put(46.33,-2){\footnotesize $t=5.39s$}
%   \put(68,36){\footnotesize Target}
%   \put(66.1,33.11){\footnotesize $n_v=20K$}
%   \put(66.1,-2){\footnotesize $t=20.8s$}
%   \put(88,36){\footnotesize Target}
%   \put(85.7,33.11){\footnotesize $n_v=150K$}
%   \put(85.7,-2){\footnotesize $t=158s$}
%   \end{overpic}
% \caption{Scalability. The vertices of the bone shapes are colored black to show the resolution (zoom in for better view), while RGB colors encode the computed map, via pull-back from the source. The corresponding runtime for our upsampling, from $5\times 5$ to $50 \times 50$ \emph{without any acceleration}, is reported below each shape.}
% \label{fig:res:eg:bones}
% \end{figure}





% \begin{figure}[!t]
% \centering
% %\includegraphics[width = 0.8\columnwidth]{figures/test_scalability_samples.pdf}
% \input{figures2/test_scalability_samples.tex}
% \caption{Acceleration strategy of sub-sampling for a pair of bones, where the source has 20K vertices, and the target has 5K vertices. We sub-sample the source shape and apply our method for refinement. The corresponding runtime and average error w.r.t. the sampling size are reported. We can see that having less than 100 samples on a 20K mesh is enough to produce a refined map with similar quality to that of our method without sampling (whose average is shown as dashed black)}.
% \label{fig:res:eval:subsampling}
% \end{figure}



% \begin{figure}[!h]
% \centering
% \begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=0.80\columnwidth]{./figures/eg_evalSmooth_maps_new.png}
% \put(11,23.1){\footnotesize Source}
% \put(34,23.1){\footnotesize Initialization}
% \put(62,23.1){\footnotesize ICP$_{30}$}
% \put(85,23.1){\footnotesize \textbf{Ours}}
% \end{overpic}
% \input{figures2/eg_evalSmooth_dirichlet.tex}
% \caption{We visualize the Dirichlet energy of the maps between a pair of horse shapes, starting with a computed functional map of size $10$ and refined either using ICP in different dimensions or using our approach until $100 \times 100$. Note that our method converges to a smoother map, whose Dirichlet energy is closer to that of ground truth.}
% \label{fig:res:eval:smoothness}
% \end{figure}



% \begin{figure}[!t]
% \centering
% %\includegraphics[width = 1.0\columnwidth]{figures/test_scalability_runtime.pdf}
% \input{figures2/test_scalability_runtime.tex}
% \caption{Scalability and accuracy test on 6 pairs of bones. The source shape has 5K vertices, and we test  different refinement techniques for the same target shape with different resolution (with the number of vertices ranging from 1K to 20K). Dashed (resp. solid) curves show the correspondence error (resp. time) of the three methods depending on the resolution.}
% \label{fig:res:eval:scalability}
% \end{figure}





%-------------- old stability figure    
% \begin{figure}[!h]
% \centering
% %\includegraphics[width = 1\columnwidth]{figures/eg_stability_v2.png}
% \input{figures2/eg_stability.tex}
% \caption{\label{fig:res:eg:stability}Stability test: given an initial $4\times 4$ functional map, we add white noise to it and use our method to refine the perturbed functional map. Here we plot the average errors of the pointwise maps over the iterations of 100 independent tests. We can observe that our method can filter out the introduced noise, typically after 8 iterations and converges to the same solution in 94 of the 100 test runs.}
% \label{fig:res:eval:stability}
% \end{figure}




%------------------------------ old version (refinement on remeshed FAUST/TOSCA)----------------------------------------------------
% \begin{figure*}[!t]
% \centering
% \input{figures2/Err_FAUST100_WKSini_direct.tex}
% \input{figures2/Err_FAUST200_WKSini_direct.tex}
% \input{figures2/Err_FAUST300_SEGini_direct.tex}
% \input{figures2/Err_TOSCAIso_WKSini_direct.tex}
% \caption{Shape matching on the FAUST and TOSCA datasets. We used~100 shape pairs for each of the three categories of the FAUST dataset and~284 pairs for the TOSCA Isometric dataset. The plots show the distribution of the {\em direct geodesic error} averaged over all the pairs.}
% \label{fig:res:refine:summary}
% \end{figure*}

% We applied our technique to refine maps between pairs of shapes in several challenging
% benchmarks and compared our method with recent state-of-the-art techniques. For reference, we used
% the evaluation datasets and baselines provided by \cite{ren2018continuous}. The datasets include the
% standard FAUST \cite{FAUST} and TOSCA \cite{TOSCA}, but where each shape is remeshed independently so that
% shapes have different number of vertices and often significantly different triangulations. As such,
% these are more challenging than the original datasets on which near-perfect results
% have been reported in the past. In all settings we initialize the maps using the standard functional
% map optimization procedure used in \cite{ren2018continuous} with the same descriptors and
% parameters. We also only allow direct maps, so that correspondences mapping left to right are
% penalized in this case, and report results with other metrics in the supplementary material. 

% Figure \ref{fig:res:refine:summary} shows the error plots for both FAUST and TOSCA datasets with automatic
% descriptor-based initialization using either WKS descriptors (WKSini) or segment-based correspondences \cite{kleiman2018robust} with the same parameters as in
% \cite{ren2018continuous}. The results shown in Figure~\ref{fig:res:refine:summary} are therefore directly comparable to the state-of-the-art results reported in \cite{ren2018continuous}. Note that in that work, BCICP
% refinement was shown to be significantly superior to the original ICP-based refinement of \cite{ovsjanikov2012functional}. In all of our experiments, we initialized the input functional map to
% be of size $20 \times 20$, which was then up-sampled to $200 \times 200$ using our method. We also compared with the recent map deblurring and denoising method \cite{ezuz2017deblurring} and with the Product Manifold Filter-based refinement
% \cite{vestner2017efficient} using the same input correspondence. As shown in Figure \ref{fig:res:refine:summary}, our
% approach achieves higher or comparable accuracy to state-of-the-art on these datasets. Perhaps more
% importantly, our method is much simpler to implement than the state-of-the-art methods. For example, BCICP explicitly refines the smoothness, coverage, bijectivity, and outlier regions using separate algorithm components for each of these four tasks.

% Figure \ref{fig:res:eg:faust_refinement} also shows a qualitative comparison with other methods on a single FAUST pair using WKS descriptors. In addition to ICP and BCICP we also experimented with an iterative version of the deblurring method of
% \cite{ezuz2017deblurring}, named ``deblur($\times 10$)``. In our experiments, however, such iterative versions did not result in
% significant improvement, as shown in Figure \ref{fig:res:eg:faust_refinement}.

%----------------------------------------------------------------------------------

%\begin{figure*}[!t]
%\centering
%\includegraphics[height = 0.22\linewidth]{figures/eg_refinement_faust_maps.png}\hspace{0.15cm}
%\input{figures2/eg_refinement_faust_curve.tex}
%\includegraphics[width = 2\columnwidth]{figures/eg_refinement_faust_v2.png} % old fig
%\caption{Refinement example. Given the initialization computed from WKS descriptors, we compare our method %with the existing refinement techniques. The runtime for our algorithm on this pair is 15s while it takes %5min for the BCICP.}
%\label{fig:res:eg:faust_refinement}
%\end{figure*}



%\myparagraph{Robustness to different surface representations.}
% We evaluate our method with respect to significant changes in surface representation. We exploit our refinement in some challenging settings for shape matching: (1) Meshes with significantly different connectivity. (2) Surfaces represented by point clouds. (3) Meshes with strong non-uniform sampling density.



% \begin{figure}[bt]
%   \centering
%   \input{./figures/FARMres.tikz}
%   \input{./figures/PCres.tikz}
%   \caption{\label{fig:FARMandPC}{\em Left}: Comparison on the FARM dataset. {\em Right}: Results on point clouds.
%   Average geodesic error on FARM: Ini$_{20}=0.0908$; ICP$_{20}=0.07944$; Fmap$_{100}=0.08429$; ICP$_{100}=0.0908$; Ours$_{100}=0.02626$. Average Euclidean error on Point Clouds: Ini$_{15}=0.05981$; ICP$_{15}=0.03539$; Fmap$_{100}=0.05319$; ICP$_{100}=0.04371$; Ours$_{100}=0.02779$.}
% \end{figure}
%




%
% \begin{figure}[!t]
% \centering
% \begin{overpic}[trim=1cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{./figures/SHREC_pair4_31_bcicp_vs_zoomOut_v2.png}
% \put(2,59){\footnotesize Source: $n_k = 53K$}
% \put(2,28){\footnotesize Target: $n_k = 16K$}

% \put(33,59){\footnotesize BCICP (500)}
% \put(33.5,28){\footnotesize Ours (500)}


% \put(57,59){\footnotesize BCICP (1000)}
% \put(58,28){\footnotesize Ours (1000)}

% \put(82,59){\footnotesize BCICP (5000)}
% \put(83,28){\footnotesize Ours (5000)}
% \end{overpic}
% \caption{Different sampling density. Here we show an example from SHREC19 dataset, where we compare our method to BCICP with different sampling density of 500, 1000, and 5000. 
% The computed maps are visualized via texture transfer and color transfer. The reference "ground-truth" map shown on the left bottom is obtained from the human body registration pipeline FARM~\cite{FARM}. From the color transfer, we can see that all the maps from ours and BCICP
% have reasonable accuracy. However, from the texture transfer, we can see that our method preserves the local details much better than BCICP. Also our method is much less dependent on the 
% sampling density than BCICP}
% \label{fig:res:shrec:bcicp_vs_zoomOut}
% \end{figure}



%%  SHREC19 summary table narrower version.
% \setlength{\tabcolsep}{0.3em}
% \begin{table}[!t]
% \caption{\textbf{SHREC19 summary}.\jing{TODO: update runtime, take transpose}}
% \label{tb:res:shrec19}
% \centering 
% \footnotesize
% \begin{tabular}{|c|c|c|c|ccc|ccc|c|c|}
% \hline
% \multirow{2}{*}{} & \multirow{2}{*}{Ini} & \multicolumn{9}{c|}{Refinement} & Improv. \\ \cline{3-12} 
%  &  & ICP & RHM & \multicolumn{3}{c|}{PMF} & \multicolumn{3}{c|}{BCICP} & Ours & Ours \\ \hline
% \#samples & - & - & - & 500 & 1000 & 5000 & 500 & 1000 & 5000 & 500 & 500 \\ \hline
% Avg. Err & 60.4 & 47.0 & 42.6 & 56.2 & 51.8 & 83.2 & 40.7 & 33.6 & 30.1 & 28.8 & 4\% \\
% Avg. Time & - & xxx & xxx & 72.9 & 118.1 & 349.3 & 90.0 & 163.7 & 437.9 & 1.5 & 400 $\times$ \\ \hline
% \end{tabular}
% \end{table}

    % We normalize each of the three coordinates of the source shape. We compute the Dirichlet energy of their images mapped on the target shape through the given map. The Dirichlet energy of the map is defined as the mean value of these three energies.
    % as:
    % \begin{equation}
    %     energy = g'*W_{\M}*g.
    %     \label{eq:dirichlet}
    % \end{equation}
    % Then we take the mean of the three energies computed in this way as the Dirichlet energy of the map.
    %Here we use \em{Dirichlet energy} to quantify the smoothness of a given map $T$ which is defined as: \jing{add the definition & discussion here?}
    
    
    %
% \begin{figure}[t]
%   \centering
%   \begin{overpic}
%   [trim=0cm 0cm 0cm 0cm,clip,width=\linewidth]{figures/noniso_transfer.png}

% %  \put(4,48){\footnotesize{Fmap$_{15}$}}
%   \put(2.5,13.5){\footnotesize{original $f$}}
%   \put(35,13.5){\footnotesize{init}}
%   \put(60.5,13.5){\footnotesize{ICP}}
%   \put(87,13.5){\footnotesize{Ours}}
%   \end{overpic}
%   %\vspace{0.15cm}
  
%   \caption{\label{fig:dog_catsmall} .}
% \end{figure}
% %
%\begin{figure}[t]
  %\centering
  %\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=\linewidth]{figures/elephant.png}
%  \put(4,48){\footnotesize{Fmap$_{15}$}} 50 150 300 1000
  %\put(2.5,15){\footnotesize{original $f$}}
  %\put(24,15){\footnotesize{Init}}
  %\put(40,15){\footnotesize{${50}$}}
  %\put(57,15){\footnotesize{${150}$}}
  %\put(72.5,15){\footnotesize{${300}$}}
  %\put(89.5,15){\footnotesize{${1000}$}}
  %\end{overpic}
  %\vspace{0.15cm}
  %\caption{\label{fig:elephant} The transfer of a delta function provided by our method for increasing number of iterations. On the left the original function on the source shape. On the right the transfer results on the target shape for different number of iterations of our method.}
%\end{figure}


%
% \begin{table}[t!] 
% \begin{tabular}{|l|c|c|c|c|c|c|c|}\hline 
% \textbf{\footnotesize function} & \textbf{\footnotesize Fmap} & \textbf{\footnotesize ICP} & \textbf{\footnotesize p2p$^{\dagger}$} & \textbf{\footnotesize ICP$\tiny{_{200}}$} & \textbf{\footnotesize Prod$^{\dagger}$} & \textbf{\footnotesize Ours} & \textbf{\footnotesize Ours$^{\dagger}$} \\\hline 
%   \footnotesize{HeatKernel} & 0.73 & 0.11 & 0.09 & 0.10 & 0.11 & \textbf{0.07} & \textbf{0.07} \\\hline 
%   \footnotesize{HeatKernel$\tiny{_{200}}$} & 0.90 & 0.77 & 0.33 & 0.17 & 0.55 & \textbf{0.13} & \textbf{0.17} \\\hline 
%   \footnotesize{HKS} & 0.66 & 0.57 & 0.18 & 0.14 & 0.21 & \textbf{0.12} & \textbf{0.12} \\\hline 
%     \footnotesize{WKS} & 0.45 & 0.13 & 0.04 & 0.06 & 0.06 & \textbf{0.03} & \textbf{0.03} \\\hline 
%  \footnotesize{XYZ} & 0.63 & 0.13 & 0.09 & 0.08 & 0.12 & 0.06 & \textbf{0.05} \\\hline 
%  \footnotesize{Indicator} & 0.69 & 0.28 & \textbf{0.11} & 0.17 & 0.20 & 0.16 & 0.16 \\\hline 
%   \footnotesize{SHOT} & 0.86 & 0.81 & 0.73 & 0.72 & 0.77 & \textbf{0.71} & \textbf{0.71} \\\hline 
%   \footnotesize{AWFT} & 0.41 & 0.25 & \textbf{0.14} & 0.15 & 0.20 & \textbf{0.14} & \textbf{0.14} \\\hline 
%   \footnotesize{Delta} & 0.97 & 0.93 & 0.50 & 0.30 & 0.80 & 0.32 & \textbf{0.32} \\\hline 
% \end{tabular} 
% \caption{Results in the transfer of different classes of functions, average on $20$ pairs from FAUST dataset intra subject. Initial Fmap size is $40 \times 30$, final size is  $210 \times 200$. The methods marked with $\dagger$ are initialized with the functional maps  estimated by $ICP$.} 
% \label{gt_transfer_test_k_Tar_39} 
% \end{table} 



% \begin{figure*}[!t]
% \centering
% \includegraphics[height=0.22\linewidth]{figures/eg_refineIter_shapes.png}\hspace{-0.3cm}\input{figures2/eg_refineIter_aveErrIter.tex}\hspace{-0.25cm}\input{figures2/eg_refineIter_ErrSummary.tex}\hspace{-0.11cm}\includegraphics[height=0.22\linewidth]{figures/eg_refineIter_maps.png}
% \vspace*{-0.1cm}
% \caption{\label{fig:res:eg:tosca_iter}Refinement over iterations. Here we compare our refinement method to the regular ICP algorithm with different dimensions w.r.t. the given initial map shown in the first column. The second figure shows the average error of the pointwise map over iterations during the refinement. The third figure shows the error summary of the refined map after 15 iterations of different refinement settings. In both plots we can see that regardless of dimension, ICP gets trapped in a local minimum. The last four columns visualize the refined maps at iteration 2, 3, 5, and 10 of ICP with dimension 100 and our method. %In both plots we can see that regardless of dimension, ICP gets trapped in a local minimum.
% \vspace{-1mm}}
% \end{figure*}

==> sections/applications.tex <==
\section{Applications}



==> tables/tb_bones_runtime.tex <==
\begin{table}[]
\begin{tabular}{|c|ccccccc|}
\hline
\multirow{2}{*}{\#vtx} & \multicolumn{3}{c|}{runtime (s)} & \multicolumn{4}{c|}{average direct error ($\times 10^{-3}$)} \\ \cline{2-8} 
 & \multicolumn{1}{c}{ICP} & \multicolumn{1}{c}{BCICP} & \multicolumn{1}{c|}{\textbf{ours}} & \multicolumn{1}{c}{Ini} & \multicolumn{1}{c}{ICP} & \multicolumn{1}{c}{BCICP} & \multicolumn{1}{c|}{\textbf{ours}} \\ \hline
1k & 0.249 & 31.58 & \multicolumn{1}{c|}{1.316} & 75.9 & 62.7 & 59.3 & 27.7 \\ \hline
2k & 0.423 & 31.31 & \multicolumn{1}{c|}{2.353} & 75.5 & 83.4 & 57.5 & 27.4 \\ \hline
5k & 1.082 & 59.79 & \multicolumn{1}{c|}{5.636} & 73.8 & 76.4 & 57.5 & 26.4 \\ \hline
10k & 2.169 & 130.2 & \multicolumn{1}{c|}{11.05} & 73.7 & 74.7 & 57.3 & 26.5 \\ \hline
15k & 3.206 & 272.9 & \multicolumn{1}{c|}{17.39} & 73.9 & 60.1 & 57.2 & 26.2 \\ \hline
20k & 4.033 & 472.1 & \multicolumn{1}{c|}{22.32} & 74.1 & 58.3 & 57.2 & 26.1 \\ \hline
\end{tabular}
\caption{Scalability test on 6 pairs of bones. The source shape has 5k vertices, then we test the different refinement techniques for the same target shape with different resolution (the number of vertices ranges from 1k to 20k).}
\end{table}
